Fast Polar Decoders: Algorithm and Implementation

Polar codes provably achieve the symmetric capacity of a memoryless channel while having an explicit construction. This work aims to increase the throughput of polar decoder hardware by an order of magnitude relative to the state of the art successive-cancellation decoder. We present an algorithm, architecture, and FPGA implementation of a gigabit-per-second polar decoder.

==> tikzlibrarymux.code.tex <==
% Define default style for this node
\tikzset{every mux2 node/.style={draw,minimum width=0.6cm,minimum height=2cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux3 node/.style={draw,minimum width=0.6cm,minimum height=3cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux4 node/.style={draw,minimum width=0.6cm,minimum height=4cm,inner sep=1mm,outer sep=0pt}}

\pgfdeclareshape{mux2}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
    % Rectangle box
    %\pgfpathrectanglecorners{\southwest}{\northeast}
  }
}

\pgfdeclareshape{mux3}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0pt%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
    % Rectangle box
    %\pgfpathrectanglecorners{\southwest}{\northeast}
  }
}

\pgfdeclareshape{mux4}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.6\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0.2\pgf@y%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.2\pgf@y%
  }
  \anchor{in3}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.6\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

